Why is the Star Formation Rate Proportional to Dense Gas Mass?

One of the most profound empirical laws of star formation is the Gao-Solomon relation, a linear correlation between the star formation rate (SFR) and the dense molecular gas mass. It is puzzling how the complicated physics in star-formation results in this surprisingly simple proportionality. Using archival Herschel and Atacama Large Millimeter/submillimeter Array Observations, we derived the masses of the most massive cores ($M^{\rm max}_{\rm core}$) and masses of the gravitationally bound gas ($ M_{\rm gas}^{\rm bound}$) in the parent molecular clouds for a sample of low-mass and high-mass star-forming regions. We discovered a significant correlation $\log(M^{\rm max}_{\rm core}/M_{\odot}) = 0.506 \log(M_{\rm gas}^{\rm bound}/M_{\odot})-0.32$. Our discovered $M^{\rm max}_{\rm core}$-$M_{\rm gas}^{\rm bound}$ correlation can be approximately converted to the Gao-Solomon relation if there is (1) a constant 30% efficiency of converting $M^{\rm max}_{\rm core}$ to the mass of the most massive star ($m^{\rm max}_{\rm star}$), and (2) if SFR and $m^{\rm max}_{\rm star}$ are tightly related through $\log({\rm SFR}/(M_{\odot} {\rm yr}^{-1})) = 2.04 \log(m^{\rm max}_{\rm star}/M_{\odot})-5.80$. Intriguingly, both requirements have been suggested by previous theoretical studies (c.f. Yan et al. 2017). Based on this result, we hypothesize that the Gao-Solomon relation is a consequence of combining the following three non-trivial relations (i) SFR vs. $m^{\rm max}_{\rm star}$, (ii) $m^{\rm max}_{\rm star}$ vs. $M^{\rm max}_{\rm core}$, and (iii) $M^{\rm max}_{\rm core}$ vs. $M_{\rm gas}^{\rm bound}$. This finding may open a new possibility to understand the Gao-Solomon relation in an analytic sense.

==> archived.tex <==
%%% Some archived paragraphs to be abandoned

% A direct link between the mass of high surface density gas and the SFR has been found in both galactic clouds \citep{Kain2009,Lada2010,Heiderman2010,Evans2014} and extragalaxies \citep{Gao2004,Garcia2012}. 

% \cite{Weidner2013} shows that the observed sample of $m_{\rm max}$ is inconsistent with random sampling from a universal IMF at a 99.9 percent confidence level.

% As the most massive core is likely to be the progenitor of the most massive stellar member, here we conduct a similar test to assess whether or not the expected number of high-mass cores in a gravitationally bound gas structure differs significantly when the cores are sampled from a fixed CMF.

% The difference lies in the intercept of the linear regression, which can be interpreted as the fraction of dense gas mass to the total parental clump mass. The fraction should depend primarily on the relative resolution differences in defining the parental structure and substructures \citep{Lin2019}. 

% The significant difference in the power-law index across different spatial resolutions can be naturally explained by the higher degree of fragmentation in more massive cores. As demonstrated by \citet{Xu2024QUARKS}, most ACA fragments contain multiple dense cores when observed with higher resolution, indicating that ACA fragments are essentially clusters of dense cores. Therefore, a shallower slope (lower index) is expected in observations with sufficiently high resolution to resolve these dense cores. 

% Across a $M_{\rm clump}$ dynamic range of $10^2$--$10^5$ \msun~\citep[one-magnitude systematically larger than that in][]{Lin2019}, they find a mass scaling relation log($M_{\rm mmc}$/$M_{\odot}$) = 0.96 log($M_{\rm clump}$/$M_{\odot}$) - 1.33, where the power law index is very consistent with what has been found in \citet{Lin2019}. 

% The difference of indexes could be reconciled due to the difference of resolution: higher resolution could result in a lower mass of dense cores. 

% SFR is defined as stellar mass in formation per unit time. However, it is difficult to make a census throughout the mass range, simply because low-mass young stellar objects (YSOs) are too faint to be detected. This incompleteness at the low-mass end leads to an underestimation of the SFR. 
% A more practical and efficient approach is to link the total mass of young star clusters ($M_{\rm \star cluster}$) with the mass of the most massive star ($M_{\rm \star max}$), as the latter can be determined by the spectral-type--stellar-mass relation for OB stars \citep{Hanson1997,Weidner2010}. Retrieving 139 young star clusters, \citet{Weidner2013} have found a correlation between $M_{\rm\star max}$ and $M_{\rm\star cluster}$. By definition, SFR should be proportional to the $M_{\rm\star cluster}$, and therefore correlate with $M_{\rm\star max}$. The correlation between SFR and $M_{\rm\star max}$ corresponds to how the SFR is estimated from luminosity \citep[e.g.][]{Gao2004} because the most massive star should dominate the luminosity over the rest population in a cluster. We should remind that stars should form in dense cores \citep{Shu1987} with $<0.1$ pc and $>10^6$\,cm$^{-3}$ \citep{WT1999}. Assuming a core-to-star efficiency of approximately 30\% \citep{Matzner2000}, we can expect a mass correlation between the most massive core and the dense gas in the parental cloud.

% With 8\parcsec5 resolution (0.12 pc at 3 kpc), an APEX/SABOCA survey at 350 $\mu$m has resolved 204 massive clumps and found a nearly linear correlation with power law index of 0.96 \citep{Lin2019}. With $\sim5$\arcsec resolution (0.07 pc at 3 kpc), \citet{Xu2024QUARKS} have observed 139 massive clumps with the Atacama Compact Array (ACA) 7-m at 1.3 mm and found the power law index also to be 0.96.

% \fengwei{Taking all these correlations into consideration, the Gao-Solomon relation can be now interpreted as the correlation between the most massive core and dense gas. Since both dense gas and cores are at the initial stage of star formation (haven't convert into stars), the correlation provides an important insight towards the underlying physics of SFR--$M_{\rm dense}$ relation. In the multi-scale context of star formation, such a correlation indicates a self-regulating scenario, where the formation of cores and subsequently stars within the parent cloud is primarily driven by growth processes in a medium with limited resources \citep{Peters2011HMSF}.}

% \subsection{Method Two} \label{temp:m2}

% The second method involves deducing the temperature of dust envelopes surrounding the fragments based on clump properties, a methodology akin to recent ALMA studies \citep[e.g.,][]{Csengeri2017,Svoboda2019,Sanhueza2019,Zhang2021,Traficante2023}. In particular, \citet{Traficante2023} categorized clumps into three groups based on their $L/M$ ratio, aligning with the three evolutionary stages outlined in \citet{Molinari16LM}. For $L/M<1 L_{\odot}/M_{\odot}$, clumps remain in a pristine, pre-stellar phase, with innermost region temperatures $T < 30$ K; within the range $1L_{\odot}/M_{\odot}\leq L/M\leq10L_{\odot}/M_{\odot}$, as clumps evolve into the protostellar phase, temperatures elevate to $T\simeq30$ K. For $L/M>10L_{\odot}/M_{\odot}$, the presence of a relatively evolved protostar heats the dust envelope, potentially forming ultra-compact HII regions, resulting in temperatures notably exceeding 30 K. Notably, some fragments might exhibit temperatures even surpassing the 40 K threshold employed in clump analyses \citep{Elia2021}. However, given that mm dust emission predominantly traces relatively cold dust envelopes, we expect no substantial increase in temperature compared to the observed 1.3 mm dust emission with ALMA. Dust temperatures at these scales vary within the range $15\leq T\leq 30$ K, covering the transition from pre-stellar to intermediate-mass protostellar fragments \citep{Motte2022ALMAIMF-1}. Furthermore, mass-averaged dust temperatures within the cores identified at $\simeq2500$ AU scales in W43-MM2\&MM3 span $20\leq\mathrm{T}\leq65$ K \citep{Pouteau22}. 

% Classification of the ALMA-IMF protocluster clouds are retrieved from Table 4 in \citet{Motte2022ALMAIMF-1}: Young (Y), Intermediate (I), and Evolved (E). Their evolutionary stage is refined from that of \citet{Csengeri2017}. Similar to what has been done in \citet{Traficante2023}, we assign dust temperature $T_{\rm dust}$ of 20, 30, and 40 K to the most massive cores in the three evolutionary groups. 

==> table1.tex <==
% \startlongtable
\begin{deluxetable*}{ccc|cccc}[!ht]
\tablecaption{Parameters of the parent molecular clouds and the most massive cores
\label{tab:mass}}
\tablewidth{2pt}
\linespread{1.2}
\tablehead{
\multicolumn{3}{c}{Parental molecular clouds} & \multicolumn{4}{c}{Most massive cores} \\
\cmidrule(r){1-3} \cmidrule(r){4-7}
\colhead{Name} & \colhead{Distance} & \colhead{$M_{\rm gas}^{\rm bound}$} & \colhead{RA} & \colhead{Dec} & \colhead{Radius} & \colhead{$M_{\rm core}^{\rm max}$} \\
\colhead{} & \colhead{(pc)} & \colhead{($\times10^3$\msun)} & \colhead{(J2000)} & \colhead{(J2000)} & \colhead{(pc)} & \colhead{(\msun)}
}
% \colnumbers
\startdata
\multicolumn{7}{c}{Nearby clouds} \\
\hline
Aquila & 278$\pm{13}$ & 4.2$^{+0.8}_{-1.7}$ & 18:29:56.9 & -01:58:29.8 & 0.15 & 56.5$\pm$16.9 \\
Cham I & 210$\pm{14}$ & 0.47$^{+0.05}_{-0.05}$  & 11:06:31.9 & -77:23:43.5 & 0.18 & 23.0$\pm$6.9 \\
Lupus I  & 151$\pm{10}$ & 0.24$^{+0.04}_{-0.02}$  & 15:45:28.4 & -34:24:02.6 & 0.12 & 6.4$\pm$1.9 \\
Lupus III  & 197$\pm{13}$  & 0.28$^{+0.07}_{-0.07}$  & 16:08:48.1 & -39:07:26.9 & 0.11 & 6.4$\pm$1.9 \\
Lupus IV  & 151$\pm{10}$ & 0.28$^{+0.08}_{-0.07}$  & 16:01:34.4 & -41:52:10.4 & 0.20 & 11.0$\pm$3.3 \\
Musca  & 160$\pm{13}$ & 0.23$^{+0.07}_{-0.05}$  & 12:25:33.9 & -71:42:06.1 & 0.19 & 5.4$\pm$1.6 \\
Ophiuchus  & 128$\pm{6}$ & 0.89$^{+0.27}_{-0.15}$  & 16:26:27.8 & -24:23:51.2 & 0.10 & 14.9$\pm$4.5 \\
Orion A & 399$\pm{19}$ & 34$^{+6}_{-6}$ & 05:35:13.5 & -05:23:57.5 & 0.14 & 264.1$\pm$79.2 \\
Perseus  & 256$\pm{12}$ & 2.7$^{+0.7}_{-0.6}$  & 03:28:39.2 & +31:18:40.6 & 0.15 & 41.1$\pm$12.3 \\
Pipe  & 180$\pm{9}$ & 0.10$^{+0.04}_{-0.02}$  & 17:11:21.3 & -27:26:17.6 & 0.08 & 6.9$\pm$2.1 \\
Taurus  & 156$\pm{7}$ & 1.8$^{+0.2}_{-0.2}$  & 04:41:26.5 & +25:23:57.2 & 0.23 & 26.7$\pm$8.0 \\
\hline
\multicolumn{7}{c}{Distant and massive clouds} \\
\hline
G008.67 & 3400$\pm{300}$ & $44^{+8}_{-7}$ & 18:06:19.1 & -21:37:31.45 & 0.08 & 70.1$\pm$34.2 \\
G010.62 & 5000$\pm{500}$ & $24^{+5}_{-3}$ & 18:10:28.7 & -19:55:49.60 & 0.12 & 163.8$\pm$81.8 \\
G012.80 & 2400$\pm{200}$ & $30^{+1}_{-1}$ & 18:14:13.7 & -17:55:43.07 & 0.05 & 32.1$\pm$15.6  \\
G327.29 & 2500$\pm{500}$ & $21^{+4}_{-5}$ & 15:53:07.8 & -54:37:06.31 & 0.04 & 67.1$\pm$40.2 \\
G328.25 & 2500$\pm{500}$ & $33^{+5}_{-6}$ & 15:57:59.8 & -53:58:00.18 & 0.05 & 24.6$\pm$15.3  \\
G333.60 & 4200$\pm{700}$ & $12^{+2}_{-5}$ & 16:22:09.5 & -50:05:58.17 & 0.08 & 60.2$\pm$34.5  \\
G337.92 & 2500$\pm{500}$ & $16^{+3}_{-4}$ & 16:41:10.5 & -47:08:03.61 & 0.07 & 115.1$\pm$68.8 \\
G338.93 & 3900$\pm{1000}$ & $11^{+1}_{-1}$ & 16:40:34.2 & -45:41:36.58 & 0.04 & 50.6$\pm$35.8  \\
G351.77 & 2000$\pm{700}$ & $16^{+3}_{-4}$ & 17:26:42.5 & -36:09:17.64 & 0.05 & 140.4$\pm$86.8 \\
G353.41 & 2000$\pm{700}$ & $18^{+4}_{-4}$ & 17:30:26.1 & -34:41:46.84 & 0.04 & 15.3$\pm$9.5  \\
W43 & 5500$\pm{400}$ & $77^{+15}_{-23}$ & 18:47:47.0 & -01:54:26.56 & 0.10 & 275.0$\pm$131.0 \\
W51 & 5400$\pm{300}$ & $100^{+20}_{-20}$ & 19:23:43.9 & +14:30:34.83 & 0.11 & 323.8$\pm$143.7 \\
\enddata
\tablecomments{The properties of nearby clouds and distant massive clouds as well as their most massive cores are listed. 
%\baobab{Double check this $M_{\rm gas}^{\rm bound}$ thing.} 
$M_{\rm gas}^{\rm bound}$: the parental gravitational bound gas. RA, Dec: equatorial coordinates of the most massive core at the epoch of J2000. 
%\baobab{$M^{\rm max}_{\rm core}$ or $M^{\rm core}_{\rm max}$?} 
$M_{\rm core}^{\rm max}$: the most massive core mass. }
\end{deluxetable*}

==> table2.tex <==
\begin{deluxetable*}{c D@{+/-}D D@{+/-}D D@{+/-}D D@{+/-}D D@{+/-}D D@{+/-}D}
\tablecaption{Parameters the most massive cores from three methods}
\tablehead{
\colhead{ALMA-IMF Field} & \multicolumn{8}{c}{Method One} & \multicolumn{8}{c}{Method Two} & \multicolumn{8}{c}{Method Three}\\
\cmidrule(r){2-9} \cmidrule(r){10-17} \cmidrule(r){18-25} 
 & \multicolumn{4}{c}{T$_{\rm dust}$ (K)} & \multicolumn{4}{c}{Mass ($M_{\odot}$)} & \multicolumn{4}{c}{T$_{\rm dust}$ (K)} & \multicolumn{4}{c}{Mass ($M_{\odot}$)} & \multicolumn{4}{c}{T$_{\rm dust}$ (K)} & \multicolumn{4}{c}{Mass ($M_{\odot}$)}
}
\decimals
\startdata
G008.67 & 69.7 & 2.1 & 101.8 & 30.7 & 100.0 & 16.0 & 70.1 & 23.2 & 100.0 & 16.0 & 69.9 & 23.2 \\
G010.62 & 91.4 & 3.1 & 177.3 & 56.4 & 100.0 & 16.0 & 163.8 & 55.9 & 100.0 & 16.0 & 163.4 & 55.8 \\
G012.80 & 80.0 & 2.4 & 39.9 & 11.9 & 100.0 & 16.0 & 32.1 & 10.6 & 100.0 & 16.0 & 32.0 & 10.5 \\
G327.29 & 86.9 & 5.9 & 264.9 & 111.7 & 300.0 & 32.0 & 67.1 & 28.5 & 100.0 & 16.0 & 226.2 & 98.1 \\
G328.25 & 86.0 & 5.8 & 28.5 & 12.0 & 100.0 & 16.0 & 24.6 & 10.7 & 100.0 & 16.0 & 24.5 & 10.7 \\
G333.60 & 111.2 & 6.3 & 53.0 & 20.3 & 100.0 & 16.0 & 60.2 & 24.0 & 100.0 & 16.0 & 60.2 & 23.9 \\
G337.92 & 84.8 & 5.3 & 136.0 & 54.9 & 100.0 & 16.0 & 115.1 & 48.4 & 100.0 & 16.0 & 115.3 & 48.4 \\
G338.93 & 75.4 & 6.5 & 68.1 & 33.1 & 100.0 & 16.0 & 50.6 & 25.1 & 100.0 & 16.0 & 50.4 & 25.1 \\
G351.77 & 92.5 & 6.2 & 151.5 & 64.0 & 100.0 & 16.0 & 140.4 & 60.9 & 100.0 & 16.0 & 141.1 & 61.6 \\
G353.41 & 76.6 & 5.2 & 20.1 & 8.5 & 100.0 & 16.0 & 15.3 & 6.6 & 100.0 & 16.0 & 15.3 & 6.7 \\
W43-MM1 & 72.6 & 1.9 & 394.7 & 115.3 & 100.0 & 16.0 & 275.0 & 88.3 & 100.0 & 16.0 & 274.0 & 88.1 \\
W43-MM2 & 60.4 & 1.5 & 399.8 & 116.1 & 100.0 & 16.0 & 228.5 & 72.9 & 100.0 & 16.0 & 228.2 & 73.3 \\
W43-MM3 & 58.7 & 1.5 & 235.6 & 68.5 & 100.0 & 16.0 & 134.5 & 43.6 & 100.0 & 16.0 & 134.3 & 43.2 \\
W51-E & 98.9 & 1.9 & 1222.7 & 342.8 & 300.0 & 32.0 & 323.8 & 94.9 & 100.0 & 16.0 & 1223.7 & 381.5 \\
W51-IRS2 & 97.0 & 2.0 & 1344.5 & 376.1 & 300.0 & 32.0 & 321.8 & 94.0 & 100.0 & 16.0 & 1308.8 & 408.1
\enddata
\tablecomments{The dust temperature estimation and the most massive core mass in three methods. $1\sigma$ uncertainty is listed for uncertainty calculation. \label{tab:method}}
\end{deluxetable*}



==> table3.tex <==
% \startlongtable
\begin{deluxetable*}{cccccccccc}
% \tabletypesize{\scriptsize}
\tabletypesize{\small}
\tablewidth{4pt}
%\tablenum{1}
\tablecaption{Associated \textit{Herschel} PACS 70 $\mu$m sources with the most massive cores in the ALMA-IMF protoclusters\label{tab:match}}
\tablehead{
\colhead{ALMAIMF} & \colhead{\textit{Herschel} PACS 70 $\mu$m} & \colhead{RA} & \colhead{Dec} & \colhead{$F_{\nu}^{\rm int}$} & \colhead{$F_{\nu}^{\rm peak}$} & \colhead{$A_{\rm FWHM}$} & \colhead{$B_{\rm FWHM}$} & \colhead{PA} & \colhead{ID} \\
\hline
 & HIGAL & \colhead{deg} & \colhead{deg} & \colhead{Jy} & \colhead{MJy sr$^{-1}$} & \colhead{arcsec} & \colhead{arcsec} & \colhead{deg} & 
}
\colnumbers
\startdata
G008.67 & PB008.6695-0.3560 & 271.57937 & $-$21.625473 & 1110.0 & 163422.7 & 14.8 & 17.3 & 151.0 & 42859 \\
G010.62 & PB010.6237-0.3828 & 272.61876 & $-$19.929828 & 6371.1 & 501480.7 & 20.4 & 23.4 & 143.0 & 40568 \\
G012.80 & PB012.8050-0.1987 & 273.55578 & $-$17.928196 & 2276.9 & 374941.1 & 13.3 & 17.1 & 137.6 & 38363 \\
G327.29 & PB327.2915-0.5777 & 238.28246 & $-$54.618348 & 2264.5 & 435621.3 & 12.9 & 15.2 & 122.6 & 95891 \\
G328.25 & PB328.2546-0.5318 & 239.49920 & $-$53.966164 & 2716.4 & 412479.2 & 16.7 & 14.8 & 139.3 & 94603 \\
G333.60 & PB333.6057-0.2139 & 245.54292 & $-$50.099757 & 11083.1 & 744856.8 & 32.3 & 17.3 & 32.2 & 86423 \\
G337.92 & PB337.9157-0.4763 & 250.29305 & $-$47.133866 & 4580.2 & 606706.8 & 17.0 & 16.6 & 41.4 & 84483 \\
G338.93 & PB338.9245+0.5567 & 250.13900 & $-$45.693888 & 435.8 & 82419.2 & 12.7 & 15.6 & 12.2 & 78449 \\
G351.77 & PB351.7754-0.5366 & 261.67799 & $-$36.154287 & 7294.5 & 629539.1 & 21.8 & 20.0 & 53.1 & 63803 \\
G353.41 & PB353.4111-0.3608 & 262.61064 & $-$34.695251 & 1781.5 & 198276.9 & 17.7 & 19.0 & 39.8 & 60972 \\
W43-MM1 & PB030.8175-0.0557 & 281.94459 & $-$1.907165 & 383.2 & 74776.3 & 14.6 & 13.2 & 69.8 & 17442 \\
W43-MM2 & PB030.7029-0.0687 & 281.90383 & $-$2.015010 & 279.1 & 63489.7 & 13.5 & 12.3 & 73.5 & 17782 \\
W43-MM3 & PB030.7202-0.0824 & 281.92393 & $-$2.005909 & 586.8 & 112427.9 & 14.6 & 13.4 & 83.6 & 17743 \\
W51-E & PB049.4894-0.3881 & 290.93332 & 14.508969 & 3522.0 & 439013.7 & 18.9 & 16.0 & 115.0 & 7027 \\
W51-IRS2 & PB049.4902-0.3688 & 290.91611 & 14.518794 & 6072.2 & 698388.7 & 16.3 & 20.0 & 117.3 & 7024 \\
\enddata
\tablecomments{The columns (1) and (2) list the ALMA-IMF fields and the associated \textit{Herschel} 70 $\mu$m sources with the most massive cores. The basic measurements are retrieved from \citep{Molinari2016HiGAL} and listed in columns (3)--(9), which includes the equatorial coordinates at the epoch of J2000, the integrated flux and peak intensity of the 70 $\mu$m sources, the full width of half maximum (FWHM) of major and minor axes as well as the position angle. The column (10) lists the Hi-GAL identity number.}
\end{deluxetable*}
